Predicting Sharp and Accurate Occlusion Boundaries in Monocular Depth Estimation Using Displacement Fields

Current methods for depth map prediction from monocular images tend to predict smooth, poorly localized contours for the occlusion boundaries in the input image. This is unfortunate as occlusion boundaries are important cues to recognize objects, and as we show, may lead to a way to discover new objects from scene reconstruction. To improve predicted depth maps, recent methods rely on various forms of filtering or predict an additive residual depth map to refine a first estimate. We instead learn to predict, given a depth map predicted by some reconstruction method, a 2D displacement field able to re-sample pixels around the occlusion boundaries into sharper reconstructions. Our method can be applied to the output of any depth estimation method, in an end-to-end trainable fashion. For evaluation, we manually annotated the occlusion boundaries in all the images in the test split of popular NYUv2-Depth dataset. We show that our approach improves the localization of occlusion boundaries for all state-of-the-art monocular depth estimation methods that we could evaluate, without degrading the depth accuracy for the rest of the images.

==> discussion.tex <==
\michael{\subsection{Impact of Depth Inpainting for Ground Truth Generation}

In NYUv2, the raw depth acquired by the Kinect sensor has a lot of missing data, due to sensor limitations. Those missing data mostly occur on reflective surfaces and along occlusion boundaries. Dense depth maps in NYUv2 are thus generated using~\cite{Levin2004colorization}, using RGB images to perform inpainting of the depth image.
Without depth inpainting, training did not converge correctly. This is most likely due to the fact that the holes are mostly located close to the occlusion boundaries.}

\subsection{Network complexity}
We now try to analyze the impact of network complexity by replacing the encoder with ResNet networks with different number of layers. As shown in Figure~\ref{fig:empirical study of network complexity}, the sharpness of occlusion boundaries benefits from the increase of number of layers in the network, until a point were performance saturates.

\begin{figure}[t]
	\begin{center}
	\end{center}
	\caption{\michaelrmk{TODO: add Figure of $\epsilon_{acc}$ vs number of layers} As we add more layers to our network, the performance improves until it reaches a saturation point.}
	\label{fig:empirical study of network complexity}
\end{figure}

%Our network has a low complexity and can be trained in very short time. 
%Therefore, instead of adding more data or designing sophisticated loss functions, using our network is a simple and fast alternative to yield high performance at the same time. 
%Figure\vincentrmk{ADD?} show the time needed to training models with different number of data and their corresponding accuracy of occlusion boundaries. \vincentrmk{CAN YOU GIVE THE RUNTIME OF THE METHOD?}


